Don't Drop Dropout: Optimizing Layer Sparsity for Efficient LLM Training and Inference

Layer dropout (a.k.a. stochastic depth) has been shown to enable faster training, higher accuracy, and robustness to zero-shot layer pruning in both language and vision transformers. However, as models and datasets have scaled, dropout - particularly layer dropout - has largely disappeared from large language models (LLMs) pre-training recipes. While some prior work has reported that dropout can degrade accuracy, no comprehensive study has quantified, let alone mitigated, this effect. In this study, we show that layer dropout should be used in state-of-the-art LLM training, establishing best practices and scaling analysis for both training and post-training benefits. Concretely, with optimal layer distribution, time schedule, and optimizer hyperparameters, we observe that at the same training FLOPs layer dropout leads to lower loss. For a given number of training steps, LLMs can achieve lower or similar validation loss while saving upto 25% of training FLOPs. Moreover, layer dropout enables significant post-training optimizations, such as early exit, intermediate-layer skipping, and self-speculative decoding, yielding up to 1.5x inference speedup with negligible accuracy loss. Across more than 2400 training experiments, spanning models from 271M to 8.2B parameters and datasets up to 160B tokens, we demonstrate that these findings extend reliably to large-scale training regimes. All pre-training experiments were run on Cerebras CS-3 systems.

==> figures/20250714_early_exit_val_loss__ablate_tpp.tex <==
\begin{figure}[H]
    \centering
    \includegraphics[width=1\linewidth]{images/20250714_early_exit_val_loss__ablate_tpp.png}
    \caption{Early Exit for dense baseline as we ablate TPP.}
    \label{fig:20250714_early_exit_val_loss__ablate_tpp}
\end{figure}

==> figures/20250819_ablate_tpp___different_dropout_configs.tex <==
\begin{figure}[H]
    \centering

    %----- Top subfigure -----
    \begin{subfigure}{\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/20250819_ablate_tpp___different_dropout_configs_val.pdf}
        \caption{Validation Loss.}
        \label{fig:top}
    \end{subfigure}

    \vspace{0.5cm}  % space between the subfigures

    %----- Bottom subfigure -----
    \begin{subfigure}{\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/20250819_ablate_tpp___different_dropout_configs_val_degradation.pdf}
        \caption{Validation Loss Degradation.}
        \label{fig:bottom}
    \end{subfigure}

    \caption{Ablating TPP for fixed model size for different layer dropout configurations.}
    \label{fig:20250819_ablate_tpp___different_dropout_configs}
\end{figure}



==> figures/20250825_repeat_drop_layer_pre_row_v2.6___dropout_distriution.tex <==
\begin{figure}[H]
    \centering
    \includegraphics[width=1\linewidth]{images/20250825_repeat_drop_layer_pre_row_v2.6___dropout_distriution.pdf}
    \caption{Ablating more dropout distributions. The notation \texttt{start::step} denotes a deterministic layer dropout pattern where skipping begins at layer \texttt{start} and proceeds with a period of \texttt{step} layers. The x-axis indicates the parameter size of each model as well as the number of layers. Models trained at 20 TPP.}
    \label{fig:20250825_repeat_drop_layer_pre_row_v2.6___dropout_distriution}
\end{figure}

==> figures/20250921_ablate_tpp_pld.tex <==
% Source: /cra-614/home/mostafae/research/monolith_config_gen/mostafae/20250921_ablate_tpp_pld/plot.ipynb
\begin{figure}[H]
    \centering
    \includegraphics[width=1\linewidth]{images/20250921_ablate_tpp_pld_sweep_stochastic_layer_drop_prob_vs_val_loss_by_n_params.pdf}
    \caption{Linear Layer, Constant Schedule}
    \label{fig:placeholder}
\end{figure}

==> figures/20250927_aspect_1d_tuned_20tpp_flopsabs.tex <==
\begin{figure}[H]
    \centering
    \includegraphics[width=0.5\linewidth]{images/20250927_aspect_1d_tuned_20tpp_flopsabs.png}
    \caption{Ablating Depth to Width Ratio. Models trained at 20 TPP.\todo[inline]{TODO: Move to appendix, or remove altogether.}}
    \label{fig:20250927_aspect_1d_tuned_20tpp_flopsabs}
\end{figure}

==> figures/20251222_ablate_tpp_reverse_schedule_bs_opt.tex <==
% Source: /cra-614/home/mostafae/research/monolith_config_gen/mostafae/20251222_ablate_tpp_reverse_schedule_bs_opt/plot.ipynb
\begin{figure}[H]
    \centering
    \includegraphics[width=1\linewidth]{images/20251222_ablate_tpp_reverse_schedule_bs_opt_val_loss_vs_tpp_ablation.pdf}
    \caption{Linear Layer, Reverse Linear Schedule}
    \label{fig:placeholder}
\end{figure}

==> figures/20251222_ablate_tpp_reverse_schedule_bs_opt_val_loss_increase_vs_tpp_ablation_percentage.tex <==
\begin{figure}[H]
    \centering
    \includegraphics[width=\linewidth]{images/20251222_ablate_tpp_reverse_schedule_bs_opt_val_loss_increase_vs_tpp_ablation_percentage.pdf}
    \caption{Linear Layer, Reverse Linear Schedule.}
    \label{fig:20251222_ablate_tpp_reverse_schedule_bs_opt_val_loss_increase_vs_tpp_ablation_percentage}
\end{figure}

==> figures/2025_08_XY_mini_fixed_depth_40__coordinate_checks.tex <==
\begin{figure}[H]
    \centering

    \begin{subfigure}{0.7\linewidth}
        \centering
        \includegraphics[width=\linewidth]{images/2025_08_04_mini_fixed_depth_40__uniform_dropout.png}
        \caption{Uniform Distribution}
        \label{fig:2025_08_XY_mini_fixed_depth_40__coordinate_checks:uniform_dropout}
    \end{subfigure}

    \vspace{0.5cm}

    \begin{subfigure}{0.7\linewidth}
        \centering
        \includegraphics[width=\linewidth]{images/2025_08_12_mini_fixed_depth_40__increasing_distb_dropout.png}
        \caption{Non-Uniform (Increasing) Distribution}
        \label{fig:2025_08_XY_mini_fixed_depth_40__coordinate_checks:increasing_dropout}
    \end{subfigure}

    \caption{Coordinate Check. Frobenius norm of activations after merged residual streams from attention
and FFN blocks across a 40 layer model of increasing dropout after training step $t$, using CompleteP (that scales residuals by $\frac{L_{\text{base}}}{L}$), and different dropout scalings, $r^{l}_{\text{train}}$ for layer $l$. 1st column: $r_{\text{train}}=1$. 2nd column: $r_{\text{train}}=\frac{1}{\rho_{l}}$.} 
    \label{fig:2025_08_XY_mini_fixed_depth_40__coordinate_checks}
\end{figure}


==> figures/training_scaling_tpp_configs.tex <==
\begin{figure}[H]
    \centering
    \includegraphics[width=\textwidth]{images/20250819_ablate_tpp___different_dropout_configs_val.pdf}
    \label{fig:top}
    \caption{Ablating TPP for fixed model size and fixed FLOPs savings for different layer dropout configurations. The difference in validation loss introduced by dropout at minimum and maximum TPPs is indicated in red.}
    \label{fig:training_scaling_tpp_configs}
\end{figure}


